What Makes Quantization for Large Language Models Hard? An Empirical Study from the Lens of Perturbation

Quantization has emerged as a promising technique for improving the memory and computational efficiency of large language models (LLMs). Though the trade-off between performance and efficiency is well-known, there is still much to be learned about the relationship between quantization and LLM performance. To shed light on this relationship, we propose a new perspective on quantization, viewing it as perturbations added to the weights and activations of LLMs. We call this approach "the lens of perturbation". Using this lens, we conduct experiments with various artificial perturbations to explore their impact on LLM performance. Our findings reveal several connections between the properties of perturbations and LLM performance, providing insights into the failure cases of uniform quantization and suggesting potential solutions to improve the robustness of LLM quantization. To demonstrate the significance of our findings, we implement a simple non-uniform quantization approach based on our insights. Our experiments show that this approach achieves minimal performance degradation on both 4-bit weight quantization and 8-bit quantization for weights and activations. These results validate the correctness of our approach and highlight its potential to improve the efficiency of LLMs without sacrificing performance.

==> table/ablation.tex <==
\begin{table}[]
\centering
\scalebox{0.85}{
\begin{tabular}{lrrrrr}
\toprule
 & Acc. & Prec. & Recall & F1 & AUC \\ 
\midrule
All Auxiliary & 0.8497 & 0.8436 & 0.8294 & 0.8371 & 0.9287 \\ 
\midrule
No Auxiliary & 0.8134 & 0.8178 & 0.7938 & 0.8034 & 0.8889 \\ 
\midrule
+CPI & 0.8270 & 0.8320 & 0.8225 & 0.8277 & 0.9173 \\ 
+CPR & 0.8186 & 0.8214 & 0.8151 & 0.8183 & 0.8978 \\ 
+CL & 0.8213 & 0.8248 & 0.8214 & 0.8241 & 0.9041 \\
\midrule
-CPI & 0.8312 & 0.8326 & 0.8140 & 0.8233 & 0.9126 \\
-CPR & 0.8417 & 0.8331 & 0.8216 & 0.8273 & 0.9172 \\ 
-CL & 0.8337 & 0.8332 & 0.8163 & 0.8247 & 0.9121 \\ 
\bottomrule
\end{tabular}}
\caption{Ablation studies of auxiliary tasks. We run experiments to test different combinations of the 3 auxiliary tasks, i.e., CPI, CPR, and CL. `+' indicates to use the single auxiliary task only while `-' denotes to exempt the auxiliary task from all the three tasks. We enumerate all possible combinations of the auxiliary tasks.}
\label{table:task}
\end{table}



==> table/main_results.tex <==
\begin{table}[]
\centering
\scalebox{0.85}{
\begin{tabular}{lrrrrr}
\toprule
Methods & Acc. & Prec. & Recall & F1 & AUC \\
\midrule
LR & 0.5250 & 0.5802 & 0.5225 & 0.5499 & 0.5447 \\
DT & 0.6237 & 0.6021 & 0.6293 & 0.6154 & 0.6273 \\
NB & 0.5219 & 0.4724 & 0.5243 & 0.4970 & 0.5300 \\
RF & 0.6484 & 0.7224 & 0.6293 & 0.6727 & 0.6958 \\
GBDT & 0.5573 & 0.6115 & 0.5517 & 0.5800 & 0.5935\\ 
\midrule
PJFNN & 0.7430 & 0.7800 & 0.6931 & 0.7367 & 0.8355 \\ 
APJFNN & 0.7600 & 0.7903 & 0.7216 & 0.7499 & 0.8469 \\
JRMPM & 0.7802 & 0.7993 & 0.7426 & 0.7734 & 0.8695 \\
ResumeGAN & 0.7743 & 0.7935 & 0.7429 & 0.7669 & 0.8625 \\
PJFCANN & 0.8126 & 0.8242 & 0.8068 & 0.8162 & 0.8938 \\
BERT & 0.7675 & 0.7944 & 0.7280 & 0.7601 & 0.8552 \\ 
BERT+TAPT & 0.8042 & 0.8189 & 0.7801 & 0.7982 & 0.8865 \\ 
\midrule
WEPJM & \textbf{0.8497$^\star$} & \textbf{0.8436$^\star$} & \textbf{0.8294$^\star$} & \textbf{0.8371$^\star$} & \textbf{0.9287$^\star$} \\
\bottomrule
\end{tabular}}
\caption{Overall performance of all methods. ‘$\star$’ indicates that we accept the improvement hypothesis of our model over the best baseline at a significant test level of 0.01.}
\label{table:results}
\end{table}

==> table/nonlinear.tex <==
\begin{table*}[t]
\begin{center}
\scalebox{0.8}{\begin{tabular}{llrrrrrrrrrrrrrr}
\toprule
Quant. & Bits & \multicolumn{4}{c|}{Bloom} & \multicolumn{6}{|c|}{OPT} & \multicolumn{4}{|c}{Llama} \\
Methods & (w/a) & 560M & 1.1B & 3B & 7.1B & 350M & 1.3B & 6.7B & 13B & 30B & 66B  & 7B & 13B & 30B & 65B\\ \midrule
\multirow{2}{*}{\textit{Wiketext-2 (ppl)}}
 \\ \\
\midrule
full & 16/16 & 19.36 & 24.33 & 11.83 & 10.32 & 15.89 & 11.35 & 8.84 & 8.32 & 7.93 & 83.01  & 19.7 & 13.3 & 10.3 & 10.18 \\ \midrule
Uniform & 4/16 & 24.19 & 29.97 & 13.41 & 11.45 & 15.95 & 11.34 & 8.86 & 8.3 & 7.93 & 41.01  & 25.05 & 14.98 & 11.78 & 11.42 \\
Non uniform & 4/16 & 22.02 & 27.67 & 12.87 & 10.98 & 15.89 & 11.35 & 8.84 & 8.3 & 7.93 && 20.92 & 15.55 & 11.03 \\ \midrule
Uniform & 8/8 & 26.14 & 36.88 & 14.98 & 15.64 & 18.28 & 12.2 & 18.83 & 3300.0 & 1328.0 & 0.84 & 100.81 & 52.41 & 57.91 & 26.88 \\
Non uniform & 8/8 & 19.78 & 24.42 & 11.9 & 10.36 & 15.95 & 11.51 & 8.86 & 8.34 & 7.93 & & 22.28 & 16.14 & 12.62 & 15.13\\ \midrule
Uniform & 4/8 & 33.31 & 44.56 & 17.28 & 17.52 & 18.33 & 12.16 & 18.58 & 3352.0 & 1262.0 & & 453.5 & 75.81 & 711.0 &  \\
Non uniform & 4/8 & 22.67 & 27.72 & 12.91 & 11.03 & 15.92 & 11.49 & 8.86 & 8.32 & 7.93 & & 21.02 & 15.58 & 11.07 \\ \midrule
\multirow{2}{*}{\textit{C4 (ppl)}}
\\ \\
\midrule
full & 16/16 & 27.83 & 22.98 & 18.08 & 15.83 & 22.94 & 16.2 & 12.91 & 12.38 & 11.78 & 83.01  & 7.67 & 7.14 & 6.5 & 6.12 \\ \midrule
Uniform & 4/16 & 34.22 & 27.41 & 20.56 & 17.52 & 22.98 & 16.2 & 12.95 & 12.38 & 11.78
 & 41.01  & 9.12 & 7.94 & 7.09 & 6.83 \\
Non uniform & 4/16 & 31.84 & 25.39 & 19.55 & 16.75 & 22.98 & 16.2 & 12.91 & 12.38 & 11.78 && 8.23 & 7.56 & 6.79\\ \midrule
Uniform & 8/8 & 34.84 & 35.81 & 21.59 & 20.64 & 26.88 & 17.94 & 98.88 & 6116.0 & 2790.0 & 0.84 & 20.05 & 18.00 & 19.36 & 18.22 \\
Non uniform & 8/8 & 28.33 & 23.08 & 18.14 & 15.89 & 22.98 & 16.42 & 12.95 & 12.4 & 11.78 & & 7.68 & 7.16 & 6.52 & 6.13 \\ \midrule
Uniform & 4/8 & 43.44 & 45.19 & 25.09 & 22.8 & 26.92 & 17.86 & 100.81 & 6116.0 & 2812.0 & & 39.09 & 28.94 & 30.39 & 28.05 \\
Non uniform & 4/8 & 32.53 & 25.48 & 19.62 & 16.81 & 22.98 & 16.42 & 12.95 & 12.38 & 11.78 & & 8.26 & 7.58 & 6.81 \\ \midrule

\multirow{2}{*}{\textit{Lambada (accuracy)}}
\\ \\
\midrule
full & 16/16 & 64.59 & 69.40.& 73.98 & 77.39 & 67.57 & 75.35 & 81.25 & 80.71 & 81.99 & 83.01  & 88.58 & 89.42 & 90.31 & 90.82 \\ \midrule
Uniform & 4/16 & 58.08 & 65.00 & 72.85 & 76.69 & 63.50 & 59.01 & 75.19 & 77.28 & 69.89 & 41.01  & 85.77 & 87.06 & 88.09 & 88.77 \\
Non uniform & 4/16 & 61.88 & 68.27 & 71.68 & 76.96 & 64.37 & 70.79 & 79.22 & 79.44 & 80.55 && 87.08 & 88.64 & 89.98\\ \midrule
Uniform & 8/8 & 59.77 & 61.90 & 68.62 & 66.87 & 64.61 & 72.91 & 41.75 & 5.38 & 3.37 & 0.84 & 86.03 & 84.10 & 65.00 & 80.45 \\
Non uniform & 8/8 & 64.70 & 68.99 & 73.77 & 77.39 & 67.65 & 74.76 & 80.94 & 80.47 & 81.84  & & 88.52 & 89.46 & 90.37 & \\ 
\bottomrule
\end{tabular}}
\end{center}
\caption{Evaluation results on Lambada.}
\label{tab:1}
\end{table*}



==> table/statistics.tex <==
\begin{table}[]
\begin{tabular}{lr}
\toprule
Statistics                             & Values \\
\midrule
\# of job postings                     & 82,362  \\
\# of resumes                          & 33,285  \\ 
\# of work experiences in resumes                 & 117,780 \\ 
avg \# of work experiences per resume & 3.57   \\
avg \# of sentences per job posting/resume & 11.83/19.75   \\
avg \# of words per job posting/resume &   114.68/258.50 \\
\# of positive person-job pairs    & 119,031  \\
\# of negative person-job pairs    &   359,721 \\
\bottomrule
\end{tabular}
\caption{The statistics of the dataset.}
\label{table:statistics}
\end{table}

